Inversion Circle Interpolation: Diffusion-based Image Augmentation for Data-scarce Classification

Data Augmentation (DA), i.e., synthesizing faithful and diverse samples to expand the original training set, is a prevalent and effective strategy to improve the performance of various data-scarce tasks. With the powerful image generation ability, diffusion-based DA has shown strong performance gains on different image classification benchmarks. In this paper, we analyze today's diffusion-based DA methods, and argue that they cannot take account of both faithfulness and diversity, which are two critical keys for generating high-quality samples and boosting classification performance. To this end, we propose a novel Diffusion-based DA method: Diff-II. Specifically, it consists of three steps: 1) Category concepts learning: Learning concept embeddings for each category. 2) Inversion interpolation: Calculating the inversion for each image, and conducting circle interpolation for two randomly sampled inversions from the same category. 3) Two-stage denoising: Using different prompts to generate synthesized images in a coarse-to-fine manner. Extensive experiments on various data-scarce image classification tasks (e.g., few-shot, long-tailed, and out-of-distribution classification) have demonstrated its effectiveness over state-of-the-art diffusion-based DA methods.

==> table5.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\addtolength{\tabcolsep}{-5pt}
\begin{table}[h]
\resizebox{\columnwidth}{!}{%
\def\arraystretch{1.1}
\begin{tabular}{c|l|c|l}
\hline\hline
Dataset &
  Suffixes &
  Dataset &
  Suffixes \\ \hline\hline
\multirow{10}{*}{5shot CUB} &
  standing on a tree branch. &
  \multirow{10}{*}{10shot CUB} &
  flying over water. \\
 &
  flying around flowers. &
   &
  standing on the ground. \\
 &
  standing on a post by the water. &
   &
  sitting on a rock. \\
 &
  flying over water. &
   &
  swimming in water. \\
 &
  standing on the ground. &
   &
  sitting on a bird feeder. \\
 &
  swimming in the water. &
   &
  standing on the beach near water. \\
 &
  sitting on a rock with a blue sky. &
   &
  perched on a wire with a blue sky in the background. \\
 &
  perched on a branch in a tree. &
   &
  standing on a branch with tall grass in the background. \\
 &
  flying over water with wings spread. &
   &
  flying in the sky with its wings spread. \\
 &
  perched on a tree branch. &
   &
   \\ \hline
\multirow{10}{*}{5shot Aircraft} &
  parked on the runway. &
  \multirow{10}{*}{10shot Aircraft} &
  flying in the sky with landing gear down. \\
 &
  flying in the sky with the landing gear down. &
   &
  taking off from the airport with a city in the background. \\
 &
  landing with another plane in the background. &
   &
  at the tarmac of an airport with a building in the background. \\
 &
  on the runway at an airport. &
   &
  with passengers, flying in the sky. \\
 &
  on the tarmac with mountains in the background. &
   &
  propeller plane on a runway, with a Honeywell sign in the background. \\
 &
  flying in the air with the landing gear down. &
   &
  airplane where workers are seen working on it in a hangar. \\
 &
  parked in a hangar with the door open. &
   &
  plane with a green stripe on the runway. \\
 &
  flying in the sky with palm trees in the background. &
   &
  with people on board, floating in water. \\
 &
  flying in the sky against a blue background. &
   &
  with a red cross on its tail and landing gear. \\
 &
  lined up on the runway at the airport. &
   &
  jet on the runway with smoke coming out of it. \\ \hline
\multirow{9}{*}{5shot Pet} &
  lying on a pillow on the floor. &
  \multirow{9}{*}{10shot Pet} &
  laying down in the grass. \\
 &
  playing with a toy on the floor. &
   &
  sitting on brown leather furniture. \\
 &
  in the grass, looking at the camera with a leash. &
   &
  sitting on a couch with a dark background. \\
 &
  on a window sill looking out. &
   &
  playing with a ball in the grass. \\
 &
  sitting on a couch with a stuffed animal. &
   &
  sitting on a windowsill, looking outdoors. \\
 &
  on a rock beside a person. &
   &
  standing on a wooden deck. \\
 &
  running in the grass with a frisbee. &
   &
  sitting inside a cage. \\
 &
   &
   &
  sitting on a chair with its mouth open. \\
 &
   &
   &
  laying on a couch with a white background. \\ \hline
\multirow{10}{*}{5shot Car} &
  parked on a city street. &
  \multirow{10}{*}{10shot Car} &
  parked on a road. \\
 &
  on a white background. &
   &
  parked on a gravel road. \\
 &
  parked in a lot with green trees in the background. &
   &
  parked with trees in the background. \\
 &
  parked on a gravel road with mountains in the background. &
   &
  driving down a forested road. \\
 &
  driving down a tree-lined road. &
   &
  driving on a dirt road in desert area. \\
 &
  parked on a black floor. &
   &
  on display at a show. \\
 &
  with its doors open. &
   &
  driving on a city street. \\
 &
  charging at a station. &
   &
  parked in a garage. \\
 &
  driving on a racing track. &
   &
  parked in front of a store with other cars. \\
 &
  driving down a rocky trail in the mountains. &
   &
   \\ \hline
\multirow{9}{*}{CUB-LT/IF=10} &
  flying over the ocean. &
  \multirow{9}{*}{Flower-LT/IF=10} &
  with water droplets on it. \\
 &
  sitting on a rock by the water. &
   &
  growing in a garden. \\
 &
  standing in the grass. &
   &
  in a close-up view. \\
 &
  flying in the sky with its wings spread. &
   &
  with a bee on it. \\
 &
  swimming in the water. &
   &
  in front of a water body. \\
 &
  standing on a sandy beach. &
   &
  against a brick wall. \\
 &
  sitting on a wire fence. &
   &
  with a butterfly on it. \\
 &
  perched on a bird feeder in the snow. &
   &
  with mixed colors in a bush. \\
 &
  standing on a tree stump. &
   &
   \\ \hline
\multirow{10}{*}{CUB-LT/IF=20} &
  sitting on a rock in the water. &
  \multirow{10}{*}{Flower-LT/IF=20} &
  close-up with a dark background. \\
 &
  perched on a branch in a tree. &
   &
  blooming in a garden. \\
 &
  standing on the ground in the grass. &
   &
  growing in a pot. \\
 &
  sitting on a post by the water. &
   &
  floating on water in a pond. \\
 &
  standing on a ledge near the water. &
   &
  arranged on a table. \\
 &
  flying in the sky with its wings spread. &
   &
  with a bee on it in the garden. \\
 &
  sitting on a branch with a blurred background. &
   &
  on a tree. \\
 &
   &
   &
  in a field with a rocky surface. \\
 &
   &
   &
  against a blue sky. \\
 &
   &
   &
  with a blurry background in a field. \\ \hline
\multirow{9}{*}{CUB-LT/IF=100} &
  flying in the sky with its wings spread. &
  \multirow{9}{*}{Flower-LT/IF=100} &
  with water droplets on it. \\
 &
  standing on the ground in the dirt. &
   &
  growing in a garden. \\
 &
  sitting on a branch of a tree. &
   &
  in a close-up view. \\
 &
  swimming in the water. &
   &
  with a bee on it. \\
 &
  perched on a hand in a grassy field. &
   &
  in front of a water body. \\
 &
  standing on the shore of the water. &
   &
  against a brick wall. \\
 &
  sitting on a branch of a tree. &
   &
  with a butterfly on it. \\
 &
  sitting on a ledge by water. &
   &
  with mixed colors in a bush. \\
 &
  standing in the water with its reflection. &
   &
   \\ \hline\hline
\end{tabular}%
}
\caption{Suffiexes of datasets.}
\label{table:5}
\end{table}
\addtolength{\tabcolsep}{5pt}


==> table6.tex <==
\begin{wrapfigure}{r}{0.34\linewidth}
\begin{minipage}{0.32\columnwidth}
\resizebox{1\columnwidth}{!}{%
\def\arraystretch{1.2}
\begin{tabular}{ccccc}
\hline
\hline

\multicolumn{1}{c}{II} & TD & \small{CLIP Score $(\uparrow)$} & \small{LPIPS $(\uparrow)$} & \small{Acc $(\uparrow)$}  \\ \hline
                      &   & \textbf{30.73}      & 47.9$\%$ & +2.11 \\
\checkmark                      &   & 30.65      & 51.5$\%$ & +3.86 \\
                      & \checkmark  & 30.63      & 50.0$\%$ & +4.15 \\
\cellcolor{mygray}\checkmark                      & \cellcolor{mygray}\checkmark  & \cellcolor{mygray}30.60      & \cellcolor{mygray}\textbf{52.7$\%$} & \cellcolor{mygray}\textbf{+5.52} \\ \hline\hline
\end{tabular}%
}
\vspace{-1em}
\captionof{table}{\textbf{Components Ablation.} ``II'' is Inversion Interpolation and ``TD" is Two-stage Denosing. ``Acc'' is the increase relative to no DA.}
\label{table:6}
\end{minipage}
\end{wrapfigure}
